Leveraging Non-uniformity in First-order Non-convex Optimization

Classical global convergence results for first-order methods rely on uniform smoothness and the \L{}ojasiewicz inequality. Motivated by properties of objective functions that arise in machine learning, we propose a non-uniform refinement of these notions, leading to \emph{Non-uniform Smoothness} (NS) and \emph{Non-uniform \L{}ojasiewicz inequality} (N\L{}). The new definitions inspire new geometry-aware first-order methods that are able to converge to global optimality faster than the classical $\Omega(1/t^2)$ lower bounds. To illustrate the power of these geometry-aware methods and their corresponding non-uniform analysis, we consider two important problems in machine learning: policy gradient optimization in reinforcement learning (PG), and generalized linear model training in supervised learning (GLM). For PG, we find that normalizing the gradient ascent method can accelerate convergence to $O(e^{-t})$ while incurring less overhead than existing algorithms. For GLM, we show that geometry-aware normalized gradient descent can also achieve a linear convergence rate, which significantly improves the best known results. We additionally show that the proposed geometry-aware descent methods escape landscape plateaus faster than standard gradient descent. Experimental results are used to illustrate and complement the theoretical findings.

==> Non-uniform Smoothness/abstract.tex <==
% !TEX root = main_paper.tex

\iffalse
The paper is organized as follows,
\begin{itemize}
    \item \textcolor{red}{(a)} Non-uniform landscapes are common in machine learning objectives, including reinforcement learning (PG) and supervised learning (GLM).
    \item \textcolor{red}{(b)} A new property called ``Non-uniform Smoothness'' is satisfied by value function, and Normalized Policy Gradient (NPG) takes advantages of Non-uniform Smoothness and achieves linear convergence rates.
    \item \textcolor{red}{(c)} General optimization results and relations with Nemirovski's lower bound and $(L_0, L_1)$-smoothness.
    \item \textcolor{red}{(d)} GLM also satisfies a more general Non-uniform Smoothness, and normalized gradient achieves better results.
    \item \textcolor{red}{(e)} A general discussion of Non-uniform Smoothness and Non-uniform \L{}ojasiewicz.
\end{itemize}

\fi

\iffalse
Modern machine learning problems require advanced optimization analyses and we demonstrate the standard techniques are incapable in term of \textit{(i)} assumptions like convexity are not satisfied by most machine learning models with parameterizations; \textit{(ii)} the classic ``uniform'' type of analyses cannot characterize non-uniform landscapes. Motivated by important applications in reinforcement learning and supervised learning, we propose two non-uniform properties, i.e., the Non-uniform Smoothness (NS) and Non-uniform \L{}ojasiewicz (N\L{}) inequality, based on which we establish general optimization results we call ``non-uniform analysis''. By exploiting the non-uniform properties, our proposed generalized version of normalization breaks known lower bounds, such as $\Omega(1/t)$ lower bound for first-order convex smooth optimization. Next, we demonstrate the power of our non-uniform analysis framework in policy gradient (PG) and generalized linear models (GLMs). In PG, normalization accelerates the convergence rate to $O(e^{- c \cdot t})$ $(c > 0)$ with much cheaper computation costs than existing algorithms. In GLM, normalization also achieves linear convergence rate of $O(e^{-t})$, significantly improving the best known results. Meanwhile, we show that the proposed algorithm escapes from plateaus of landscapes much faster than standard gradient descent update. The theoretical findings are verified by experimental results.
\fi

\iffalse
% The first-order optimization is the major fuel of the successful deep learning and reinforcement learning. However, the understanding of first-order methods is still limited, which leaves many mythical observations and rules of thumb in practice. 
% In this paper, we establish general optimization framework to investigate the mythical observations and rules of thumb in first-order methods for non-convex machine learning problems, and guide the design of their acceleration. 
In this paper, we establish general optimization framework by exploiting two versatile \emph{non-uniform} geometry properties in practical problems, i.e., the Non-uniform Smoothness (NS) and Non-uniform \L{}ojasiewicz (N\L{}) inequality, which strictly generalize the global convex and smoothness in the vanilla convex optimization, respectively. 
% 
% which are versatile in many machine learning problems, to investigate the convergence of first-order methods and to guide the acceleration of the vanilla algorithms in more practical problems. 
%
% \textcolor{red}{We establish general optimization results, which shows that standard gradient descent follows convergence rate upper and lower bounds.} 
%
The non-uniform properties inspires the geometry-aware normalization in gradient descent, breaking the known lower bounds, $\Omega(1/t^2)$, in first-order convex smooth optimization. We further demonstrate the power of geometry-aware normalization and the non-uniform analysis in policy gradient (PG) in reinforcement learning and generalized linear models (GLMs) in supervised learning. In PG, normalization accelerates the convergence rate to $O(e^{- c \cdot t})$ $(c > 0)$ with much cheaper computation costs than existing algorithms. In GLM, normalization also achieves linear rate, significantly improving the best known results. Meanwhile, we show that the proposed geometry-aware algorithm escapes from plateaus of landscapes much faster than standard gradient descent update. Finally, we empirically justify the theoretical findings by experimental results.
\fi

%We present a new framework for establishing
%the global convergence of first-order methods
%in a 
%class of optimization problems that extends beyond convex.
%%broader class of optimization problems than convex.
%%
%%Our framework 
%The framework we propose
%is based on two new landscape properties,
%\emph{Non-uniform Smoothness} (NS)
%and the \emph{Non-uniform \L{}ojasiewicz inequality} (N\L{}),
%that respectively generalize the classical notions
%of global smoothness and global convexity.
Classical global convergence results for first-order methods 
rely on uniform smoothness and the
\L{}ojasiewicz inequality.
Motivated by properties of objective functions that arise in machine learning,
we propose a non-uniform refinement of these notions, leading to
\emph{Non-uniform Smoothness} (NS)
and 
\emph{Non-uniform \L{}ojasiewicz inequality} (N\L{}).
The new definitions
inspire new 
geometry-aware first-order methods that are able to
converge to global optimality faster than
%are able to achieve global optimality surpassing 
the classical $\Omega(1/t^2)$ lower bounds.
%by exploiting the more refined notions of landscape structure.
%
To illustrate the power of these geometry-aware methods
and their corresponding non-uniform analysis,
we consider two important problems in machine learning:
policy gradient optimization in reinforcement learning (PG),
and generalized linear model training in supervised learning (GLM).
%
For PG, %policy gradient optimization,
we find that normalizing the gradient ascent method
can accelerate convergence to $O(e^{- c \cdot t})$ (where $c > 0$)
while incurring less overhead than existing algorithms.
For GLM, %generalized linear model training,
we show that geometry-aware normalized gradient descent can also achieve a linear
convergence rate, which significantly improves the best known results.
%
We additionally show that the proposed geometry-aware gradient descent methods
escape landscape plateaus faster than standard gradient descent.
Experimental results are used to illustrate and complement the theoretical findings.
%The theoretical findings are further supported %by experimental results.
%experimentally.


==> Non-uniform Smoothness/acknowledgements.tex <==
\section*{Acknowledgements}

The authors would like to thank anonymous reviewers for their valuable comments. Jincheng Mei would like to thank Fuheng Cui for spotting a mistake in \cref{fig:example_power_1p5}(c) in a previous verion. Jincheng Mei would like to thank Ziyi Chen for pointing that N\L{} recovers global K\L{} property. Jincheng Mei and Bo Dai would like to thank Nicolas Le Roux for providing feedback on a draft of
this manuscript.
Csaba Szepesv\'ari and Dale Schuurmans gratefully acknowledge funding from the Canada CIFAR AI Chairs Program, Amii and NSERC.

==> Non-uniform Smoothness/conclusions_future_work.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions_future_work}

The main contributions of this paper concern a general characterization and analysis based on non-uniform properties, which are not only sufficiently general to cover concrete examples, but also significantly improve convergence rates over previous work and even over classical lower bounds. The most exciting part is the techniques apply to important applications in machine learning that involve non-convex optimization problems. One direction is to further push the analysis to other domains with more complex function approximators, including neural networks \citep{allen2019convergence}. Another valuable future work is to incorporate stochastic gradient \citep{karimi2016linear} and other adaptive gradient-based methods \citep{kingma2014adam} in the analysis. Finally, applying other cases of non-uniform properties beyond those mentioned in this paper would be interesting.

==> Non-uniform Smoothness/generalized_linear_model.tex <==
% !TEX root = main_paper.tex

%\vspace{-3mm}
\section{Generalized Linear Models}
\label{sec:generalized_linear_model}

% With the strong policy optimization results in RL established, it is natural to ask if the non-uniform analysis benefits other domains. 
Next, we investigate the generalized linear model (GLM) with quasi-maximum likelihood estimate (quasi-MLE), which applied widely in supervised learning. We show that the mean squared error (MSE) of GLM \citep{hazan2015beyond} is in the non-convex function class $\gZ$ in \cref{fig:non_uniform_function_classes_diagram_table}, and it satisfies the case (2) in \cref{thm:general_optimization_main_result_1} with $\xi = 1/2$. As a result, both GD and GNGD achieve global linear convergence rates $O(e^{-c \cdot t})$, significantly improving the best existing results of $O(1 / \sqrt{t})$ \citep{hazan2015beyond}. We also provide new understandings of using normalization in GLM based on our non-uniform analysis.

\subsection{Basic Settings and Notations}

Given a training data set $\gD = \{ ( x_i, y_i ) \}_{ i \in [N] }$, which consists of $N$ data points, there is a feature map $x_i \mapsto \phi(x_i) \in \sR^d$ for each pair $(x_i, y_i) \in \gD$. We denote $\phi_i \coloneqq \phi(x_i)$ for conciseness. For each data point $x_i$, we have $y_i \in [0, 1]$ as the ground truth likelihood. Following \citet{hazan2015beyond}, our model is parameterized by a weight vector $\theta \in \sR^d$ as ,
\begin{align}
    \pi_i = \sigmoid(\phi_i^\top \theta) = \frac{1}{1 + \exp\{ - \phi_i^\top \theta \}},
\end{align}
where $\sigmoid: \sR \to (0,1)$ is the sigmoid activation. The problem is to minimize the mean squared error (MSE),
\begin{align}
\label{eq:mean_squared_error_sigmoid}
    \min_{\theta} \gL(\theta) = \min_{\theta \in \sR^d} \frac{1}{N} \cdot \sum_{i=1}^{N}{ (\pi_i - y_i)^2 }.
\end{align}
We assume $y_i = \pi_i^* \coloneqq \sigmoid(\phi_i^\top \theta^*)$, where $\theta^* \in \sR^d$, and $\left\| \theta^* \right\|_2 < \infty$, which means the target $y_i$ is realizable and non-deterministic. According to \citet{hazan2015beyond}, the MSE in \cref{eq:mean_squared_error_sigmoid} is not quasi-convex (thus not convex). Fortunately, \citet{hazan2015beyond} manage to show that \cref{eq:mean_squared_error_sigmoid} satisfies a weaker Strictly-Locally-Quasi-Convex (SLQC) property, based on which they prove the following result:
\begin{theorem}[\citet{hazan2015beyond}]
\label{thm:ngd_glm_sigmoid_convergence_rate}
With diminishing learning rate $\eta_t \in \Theta(1/\sqrt{t})$, the normalized gradient descent (NGD) update $\theta_{t+1} \gets \theta_t - \eta_t \cdot \frac{\partial \gL(\theta_t)}{\partial \theta_t} \Big/ \left\| \frac{\partial \gL(\theta_t)}{\partial \theta_t} \right\|_2$ satisfies,
\begin{align}
    \delta(\theta_t) \coloneqq \gL(\theta_t) - \gL(\theta^*) \in O(1/\sqrt{t}),
\end{align}
where $\theta^* \coloneqq \argmin_{\theta}{ \gL(\theta) }$ is the global optimal solution.
\end{theorem}

\subsection{Fast Convergence using Non-uniform Analysis}

Based on the $O(1/\sqrt{t})$ rate for NGD in \cref{thm:ngd_glm_sigmoid_convergence_rate}, \citet{hazan2015beyond} propose to normalize gradient norm in MSE minimization. However, there is no lower bound for other methods including GD on GLM, and thus it is not clear if there exists a faster rate for GLM optimization.

Surprisingly, we prove that both GD and GNGD actually achieve much faster rates of $O(e^{-c \cdot t})$ using the non-uniform analysis. Our first key finding is to show that the MSE in GLM satisfies a new N\L{} inequality with $\xi = 1/2$:
\begin{lemma}[N\L{}]
\label{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable}
Denote $u(\theta) \coloneqq \min_{i \in [N]}{ \left\{ \pi_i \cdot \left( 1 - \pi_i \right) \right\} }$, and $v \coloneqq \min_{i \in [N]}{ \left\{ \pi_i^*\cdot \left( 1 - \pi_i^* \right) \right\} }$. We have,
\begin{align}
    \left\| \frac{\partial \gL(\theta)}{\partial \theta} \right\|_2 \ge C(\theta, \phi) \cdot \left[ \frac{1}{N} \cdot \sum_{i=1}^{N}{ \left( \pi_i - \pi_i^* \right)^2 } \right]^{\frac{1}{2}},
\end{align}
holds for all $\theta \in \sR^d$, where 
\begin{align}
    C(\theta, \phi) = 8 \cdot u(\theta) \cdot \min\left\{ u(\theta), v \right\} \cdot \sqrt{\lambda_\phi},
\end{align}
and $\lambda_\phi$ is the smallest positive eigenvalue of $\frac{1}{N} \cdot \sum_{i=1}^{N}{ \phi_i \phi_i^\top}$.
\end{lemma}
\begin{remark}
It is not clear if results similar to \cref{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable} hold without assuming: \textit{(i)} realizable optimal prediction $y_i = \pi_i^* \coloneqq \sigmoid(\phi_i^\top \theta^*)$; \textit{(ii)}  non-deterministic optimal prediction $\left\| \theta^* \right\|_2 < \infty$. We leave it as an open question to study non-uniformity of GLM without the above assumptions.
\end{remark}
In \cref{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable}, $\lambda_\phi$ is determined by the feature $\phi$, and $u(\theta)$ shows that the gradient is vanishing when $\pi_i$ is near deterministic, which is consistent with the fact that the sigmoid saturates and provides uninformative gradient as the parameter magnitude becomes large.
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figs/glm_sigmoid_non_uniform_smoothness.pdf}
%\vskip -0.1in
\caption{Experiments on GLM using GD.} 
\label{fig:glm_sigmoid_non_uniform_smoothness}
%\vskip -0.1in
\end{figure}

We run GD on one example with $N = 10$ and $d = 2$. As shown in \cref{fig:glm_sigmoid_non_uniform_smoothness}, the gradient norm $\left\| \nabla \gL(\theta_t) \right\|_2$ is close to zero at plateaus and near optimum. However, unlike the PG, the spectral radius of the Hessian $\nabla^2 \gL(\theta_t)$ is only close to zero at plateaus, while it approaches positive constant near optimum. This indicates a different NS condition other than \cref{lem:non_uniform_smoothness_softmax_special,lem:non_uniform_smoothness_softmax_general} is needed, since only gradient norm $\to 0$ cannot upper bound the spectral radius of Hessian $\to c > 0$. With some calculations, we prove the following key results:
\begin{lemma}[Smoothness and NS]
\label{lem:non_uniform_smoothness_glm_sigmoid_realizable}
$\gL(\theta)$ satisfies $\beta$ smoothness with 
\begin{align}
\beta = \frac{3}{8} \cdot \max_{i \in [N]}{ \left\| \phi_i \right\|_2^2 },   
\end{align}
and $\beta(\theta)$ NS with
\begin{align*}
    \beta(\theta) = L_1 \cdot \left\| \frac{\partial \gL(\theta)}{\partial \theta} \right\|_2 + L_0 \cdot \left( \left\| \frac{\partial \gL(\theta)}{\partial \theta} \right\|_2^2 \Big/ \gL(\theta) \right).
\end{align*}
\end{lemma}
At the optimal solution $\theta^*$, the spectral radius of the Hessian $\frac{\partial^2 \gL(\theta^*)}{\partial (\theta^*)^2}$ is strictly positive. Therefore, the MSE objective of \cref{eq:mean_squared_error_sigmoid} is in the non-convex function class $\gZ$ in \cref{fig:non_uniform_function_classes_diagram_table}, and it satisfies the case (2) in \cref{thm:general_optimization_main_result_1} with $\xi = 1/2$. Combining \cref{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable,lem:non_uniform_smoothness_glm_sigmoid_realizable} and applying \cref{thm:general_optimization_main_result_1}, we have the following global linear convergence result:
\begin{theorem}
\label{thm:final_rates_normalized_glm_sigmoid_realizable}
With $\eta = 1/ \beta $, GD update satisfies for all $t \ge 1$, $\gL(\theta_t) \le \gL(\theta_1) \cdot e^{- C^2 \cdot (t-1)}$.
With $\eta \in \Theta(1)$, GNGD update satisfies for all $t \ge 1$, $\gL(\theta_t) \le \gL(\theta_1) \cdot e^{- C \cdot (t-1)}$, where $C \in (0,1)$, i.e., GNGD is strictly faster than GD.
\end{theorem}
\cref{thm:final_rates_normalized_glm_sigmoid_realizable} significantly improves the $O(1/\sqrt{t})$ rate in \cref{thm:ngd_glm_sigmoid_convergence_rate}. The key difference is that we discovered a new N\L{} inequality of \cref{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable} that is satisfied by GLMs. The linear convergence rates are verified in \cref{sec:additional_simulations_experiments}.

In \cref{thm:final_rates_normalized_glm_sigmoid_realizable}, we have $C = \inf_{t \ge 1}{ C(\theta_t, \phi)}$, which is very close to zero if $\pi_i$ is near deterministic, and GD suffers sub-optimality plateaus as shown in \cref{fig:example_glm_sigmoid}. GNGD has strictly (orders of magnitudes) better constant dependence $C \gg C^2$, and escapes plateaus significantly faster than GD. Intuitively, for the GLM in \cref{fig:example_glm_sigmoid}, $C$ in \cref{thm:general_optimization_main_result_1} is lower bounded reasonably if $\theta_1$ is initialized within some finite distance of the central valley containing $\theta^*$.

Combining the N\L{} and NS properties (\cref{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable,lem:non_uniform_smoothness_glm_sigmoid_realizable}), we provide new understandings of using normalization in GLM: \textit{(i)} \textbf{First}, using standard NGD \citep{hazan2015beyond} for all $t \ge 1$ is not a good choice. By examining the asymptotic behaviour as $\theta \to \theta^*$, we have $\beta(\theta) \to \beta > 0$. However, the normalization $\Big\| \frac{\partial \gL(\theta)}{\partial \theta} \Big\|_2$ in standard NGD gives incremental updates with adaptive stepsize $\to \infty$. To guarantee convergence, it is necessary to use $\eta_t \to 0$, which counteracts normalization and slows down the learning, since it could be not easy to find a learning rate scheme. This is consistent with the $O(e^{-c \cdot t})$ result for GD with $\eta > 0$ and without normalization in  \cref{thm:final_rates_normalized_glm_sigmoid_realizable}. \textit{(ii)} \textbf{Second}, using geometry-aware normalization $\beta(\theta_t)$ is a better choice than normalizing the gradient norm $\left\| \nabla \gL(\theta_t) \right\|_2$. We elaborate this point by investigating \textit{both the asymptotic and the early-stage behaviours} using NS-N\L{}. Since $\beta(\theta_t) \to \beta > 0$ asymptotically, GNGD is approaching GD as $\theta_t \to \theta^*$, which makes GNGD enjoy the same $O(e^{- c \cdot t})$ rate. On the other hand, at early-stage optimization (e.g., close to initialization in \cref{fig:example_glm_sigmoid}), when $\theta_t$ is far from $\theta^*$, we have thus $\beta(\theta_t) \le c \cdot \left\| \frac{\partial \gL(\theta_t)}{\partial \theta_t} \right\|_2$. Then GNGD is close to NGD, which guarantees strictly better progresses than GD. This is because of the progress of GNGD in each iteration at this time is about $\left\| \nabla \gL(\theta_t) \right\|_2$, while the progress of GD is $\left\| \nabla \gL(\theta_t) \right\|_2^2$, and the gradient norm is close to $0$ on plateaus. Using N\L{} of \cref{lem:non_uniform_lojasiewicz_glm_sigmoid_realizable}, GNGD will have strictly better constant dependence $C$ than $C^2$ in GD.


==> Non-uniform Smoothness/introduction.tex <==
% !TEX root = main_paper.tex

%\vspace{-5mm}
\section{Introduction}
\label{sec:introduction}
% \vspace{-2mm}



The optimization of non-convex objective functions
is a topic of key interest in modern-day machine learning.
Recent, intriguing results show that
simple gradient-based optimization can achieve \emph{globally} optimal solutions in certain 
non-convex problems arising in machine learning,
such as in reinforcement learning~(RL) \citep{agarwal2020optimality}, supervised learning~(SL) \citep{hazan2015beyond}, and deep learning \citep{allen2019convergence}.
While gradient-based algorithms remain the method of choice in machine learning, 
the convergence of such algorithms to global minimizers has still only been established in restrictive settings where one can assert two strong assumptions about the objective function:
(1) that the objective is smooth,
and (2) that the objective satisfies a gradient dominance over sub-optimality such as the \L{}ojasiewicz inequality. We will find it beneficial to recall the definitions of these properties. For the remainder of this paper let $\Theta = \R^d$. % and the functions $f: \Theta \to \R^d$ will be taken to be differentiable.

\begin{definition}[Smoothness]
\label{def:smoothness}
The function $f: \Theta \to \sR$ is $\beta$-smooth ($\beta > 0$) if it is differentiable and 
for all $\theta,\theta^\prime \in \Theta$,
\begin{align}
%\textstyle
    \left| f(\theta^\prime) - f(\theta) - \Big\langle \frac{d f(\theta)}{d \theta}, \theta^\prime - \theta \Big\rangle \right| \le \frac{\beta}{2} \cdot \| \theta^\prime - \theta \|_2^2.
    \label{eq:uniform smoothness}
\end{align}
\end{definition}

\begin{definition}[]%\L{}ojasiewicz inequality
\citep{lojasiewicz1963propriete,polyak1963gradient,kurdyka1998gradients} %]
\label{def:lojasiewicz}
The differentiable function $f: \Theta \to \sR$ satisfies the $(C, \xi)$-\L{}ojasiewicz inequality if for all $\theta \in  \Theta$,
\begin{align}
%\textstyle
    \left\| \frac{d f(\theta)}{d \theta} \right\|_2 \ge C \cdot \Big( f(\theta) - \inf_{\theta \in \Theta}{ f(\theta) } \Big)^{1 - \xi},
    \label{eq:lojasiewicz}
\end{align}
where $C > 0$ and $\xi \in [0, 1]$.
\end{definition}

In particular, if an objective function $f$ satisfies both assumptions, gradient-based optimization can be shown to converge to a global minimizer by noting first that uniform smoothness \cref{eq:uniform smoothness} ensures the gradient updates achieve monotonic improvement with an appropriate step size (i.e., $f(\theta_{t+1}) \le f(\theta_t) - \frac{1}{2 \beta} \cdot \left\| \nabla f(\theta_t) \right\|_2^2$, if $\theta_{t+1} \gets \theta_t - \frac{1}{\beta} \cdot \nabla f(\theta_t)$),
while the \L{}ojasiewicz inequality \cref{eq:lojasiewicz} ensures the gradient does not vanish before a global minimizer is reached.
Several global convergence results have recently been achieved in the machine learning literature by exploiting assumptions of this kind. 
For example, in reinforcement learning it has recently been shown that policy gradient (PG) methods converge to a globally optimal policy \citep{agarwal2020optimality,mei2020global};
in supervised learning it has been shown that gradient descent (GD) methods converge to global minimizers of certain non-convex problems \citep{hazan2015beyond};
and in deep learning theory it has been shown that (stochastic) GD can converge to a global minimizer with an over-parameterized neural network \citep{allen2019convergence}. 

However, previous work that relies on the two \emph{uniform} conditions in \cref{def:smoothness,def:lojasiewicz} assumes \emph{universal constants} $\beta$ and $C$, which ignores important problem structure and limits both the applicability of the results and the strength of the results that can be obtained. 


%%%% motivation was here, moved to motive.tex

In this paper, we expand the class of problems for which gradient-based optimization is globally convergent, 
develop novel gradient-based methods that better exploit local structure,
and improve the convergence rate analysis. 
We achieve these results by first defining then investigating a new set of \emph{non-uniform}
%
%Motivated by practical problems in deep learning \citep{zhang2019gradient}, RL \citep{mei2020global}, and SL \citep{hazan2015beyond}, 
%In particular,
%we study non-uniform properties of 
smoothness and \L{o}jasiewicz inequalities,
which generalize the classical definitions and allow a refined characterization of the space of objectives.
Given these refined notions,
we then tailor novel gradient-based algorithms that improve previous methods for these new problem classes,
%We introduce new non-uniform characterization, which categorizes the optimizations, and establish analysis 
and extend the analysis to exploit these new forms of non-uniformity, achieving significantly stronger convergence rates in many cases.
Importantly, these improvements are achieved in non-convex optimization problems that arise in relevant machine learning problems.
%apply to important applications in RL and SL. More importantly, from the new analysis we derive novel algorithms that achieve stronger rates than existing results. We summarize our contributions as follows.

\iffalse
\textit{First}, we formally propose two core concepts, i.e., the Non-uniform Smoothness (NS) property, and the Non-uniform \L{}ojasiewicz (N\L{}) inequality. The N\L{} inequality not only recovers  (strong) convexity as special cases, but also apply to non-convex functions in reinforcement learning and supervised learning. The NS property provides a general principled way to characterize the non-uniform objective landscapes. Based on these non-uniform properties, we then establish non-uniform analyses, which show that GNGD $(1)$ enjoys strictly faster global convergence rates than GD when the global optimum is not first-order strict optimum; $(2)$ enjoys strictly faster escaping plateaus than GD and strictly faster convergence rates than standard normalized gradient descent (NGD) \citep{nesterov1984minimization,hazan2015beyond}; $(3)$ achieves faster rates than existing lower bound results in optimization literature. The reason of why $(3)$ happens is further explained by subdividing the smooth function class, which is realizable after introducing the new NS property.

\textit{Second}, we apply our non-uniform analysis to reinforcement learning. In particular, we show that $(1)$ with softmax parameterization, the policy value satisfies the NS property, and the global optimal policy is not a first-order strict optimum; $(2)$ NPG escapes from plateaus near deterministic sub-optimal policies strictly faster than standard policy gradient method; and $(3)$ the Normalized Policy Gradient (NPG) method enjoys global linear $O(e^{-t})$ convergence rate, without using regularization (which changes the original objective) or expensive updates like line-search and natural gradient. The result largely improves existing rates~\citep{agarwal2020optimality} and is faster than the $\Omega(1/t)$ lower bound of standard policy gradient methods \citep{mei2020global}. 

\textit{Third}, we apply our non-uniform analysis in supervised learning and show that $(1)$ the Generalized Linear Model (GLM) objective with sigmoid activation satisfies the N\L{} inequality and NS property; $(2)$ GNGD escapes from the plateaus strictly faster than GD; $(3)$ GNGD enjoys global linear convergence rate $O(e^{-t})$, which significantly improves over the existing $O(1/\sqrt{t})$ result of normalized gradient descent (NGD) \citep{hazan2015beyond}. 
\fi

The remainder of the paper is organized as follows.
First, in \cref{sec:motivation} we illustrate how natural optimization problems, including those in machine learning, exhibit interesting \emph{local} structure that cannot be adequately captured by the
%can be  exploited to significantly strengthen these prior results.
%First, in \cref{sec:motivation} we provide a concrete explanation of the shortcoming of using 
uniform smoothness and \L{}ojasiewicz inequalities.
%, and explain how these can neglect critical problem structure.
Then, \cref{sec:non_uniform_propterties} introduces the 
%NS property and the N\L{} inequality, 
the Non-uniform Smoothness (NS) property and the Non-uniform \L{}ojasiewicz (N\L{}) inequality,
based on which \cref{sec:non_uniform_analysis} provides non-uniform analyses. \cref{sec:policy_gradient,sec:generalized_linear_model} then present new results for policy gradient and generalized linear models respectively. \cref{sec:conclusions_future_work} concludes the paper and discusses some future directions. 
Due to space limits, we relegate most of the proofs to the appendix. 

\if0

We have $f$ is convex but not strongly convex, since $f^{\prime\prime}(x) = 12 \cdot x^2 \ge 0$ and $f^{\prime\prime}(x)$ is arbitrarily close to $0$ when $x$ is close to $0$. Therefore, using a universal constant $\beta$ to upper bound $f^{\prime\prime}(x)$ everywhere is too coarse. A natural question is whether it benefits optimization if we use more sophisticated landscape characterization? Simulations show promising evidences.
\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{figs/example_power_4.pdf}
\vskip -0.1in
\caption{Two updates on $f: x \mapsto x^4$.} 
\label{fig:example_power_4}
\vskip -0.2in
\end{figure}

We compare the convergence rates of two updates in terms of sub-optimality $\delta(x_t) \coloneqq x_t^4$, as shown in \cref{fig:example_power_4}. The standard gradient descent (GD): $x_{t+1} \gets x_t - \eta \cdot f'(x_t)$ achieves sublinear rate about $O(1/t^2)$, while another update we call Geometry-aware Normalized GD (GNGD): $x_{t+1} \gets x_t - \eta \cdot f'(x_t) / \left\| f'(x_t) \right\|_2^{2/3}$ enjoys linear rate $O(e^{-t})$.

Two questions arise from the results, (1) GD on convex smooth function achieves $O(1/t)$ rate \citep{nesterov2003introductory}, while in subfigure(b) the rate is about $O(1/t^2)$; (2) GNGD achieves $O(e^{-t})$, which is faster than the $\Omega(1/t^2)$ lower bound \citep{nemirovski1983problem}.

\fi

==> Non-uniform Smoothness/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{amssymb,amsthm}
\usepackage{mathtools}
\usepackage{algorithm,algorithmic}
\usepackage{natbib}
\usepackage{xcolor}
\usepackage{hyperref}
\usepackage{url}
\usepackage{cancel}
%\usepackage{etoc}
\usepackage[capitalize]{cleveref}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\crefname{proposition}{Proposition}{Propositions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{update_rule}{Update}{Updates}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{figure}{Figure}{Figures}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}


\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}
\newtheorem{update_rule}{Update}
\newtheorem{claim}[theorem]{Claim}


\DeclareMathOperator*{\expectation}{\mathbb{E}}
\def\rvpi{{\boldsymbol{\pi}}}
\def\rvdelta{{\boldsymbol{\delta}}}
\def\rvtheta{{\boldsymbol{\theta}}}
\def\rvTheta{{\boldsymbol{\Theta}}}

\def\rvone{{\mathbf{1}}}
\def\rvzero{{\mathbf{0}}}

\def\identitymatrix{\mathbf{Id}}
\def\diagonalmatrix{\text{diag}}
\def\linearspan{\text{Span}}

\DeclareMathOperator*{\subjecto}{subject\,to}
\DeclareMathOperator*{\probability}{Pr}

\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}

\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}


==> Non-uniform Smoothness/motive.tex <==
%!TEX root = main_paper.tex
\section{Motivation}
\label{sec:motivation}

To illustrate the significance of non-uniformity in %global optimization, 
machine learning problems,
we consider examples motivated by recent theoretical \citep{zhang2019gradient,wilson2019accelerating,mei2020global} and empirical studies \citep{cohen2021gradient}.

Regarding smoothness, it is clear that a uniform smoothness constant $\beta$ cannot always adequately characterize an objective over its entire domain.
For example, the convex function $f:x\mapsto x^4$ cannot be informatively characterized by a uniform smoothness constant $\beta$
because its Hessian $f^{\prime\prime}:x \mapsto 12 \cdot x^2$ has the property that
$f^{\prime\prime}(x)\to\infty$ as $|x|\to\infty$, and $f^{\prime\prime}(x)\to0$ as $|x|\to0$. 
Varying smoothness of this kind has motivated the study of alternative definitions to explain, for example, the effectiveness of gradient clipping in training neural networks and normalization in optimization \citep{zhang2019gradient,wilson2019accelerating}.
Meanwhile \citet{cohen2021gradient} present neural network training results that cannot be well explained using the standard smoothness condition of \cref{def:smoothness}. 

Regarding the \L{}ojasiewicz inequality, a recent study of policy gradient optimization in reinforcement learning has shown that,
with the standard softmax parameterization, the expected return objective cannot satisfy \emph{any} \L{}ojasiewicz inequality with a universal constant $C$ \citep{mei2020global}, which 
removes the possibility of using \cref{def:lojasiewicz} to prove convergence.
By introducing a \emph{non-uniform} version of the \L{ojasiewicz} inequality, the same authors were able to show a global convergence rate for the same problem.

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figs/glm_sigmoid_example.pdf}
%\vskip -0.1in
\caption{Non-uniform landscape of non-convex function.}
\label{fig:example_glm_sigmoid}
%\vskip -0.15in
\end{figure}

\cref{fig:example_glm_sigmoid} illustrates another example of a  non-convex objective, which arises in supervised learning. Subfigure 1(a) visualizes the mean squared error (MSE) of a generalized linear model (GLM) \citep{hazan2015beyond}, which is not only non-convex but also highly non-uniform. 
As a ``teaser'', subfigure 1(b) compares the convergence behavior of two algorithms: standard gradient descent (GD), which suffers from slow convergence on the plateaus due to the non-uniformity of the objective, and an alternative algorithm (GNGD), soon to be introduced. 
This figure previews how proper handling of non-uniformity in the optimization landscape can enable significant acceleration of optimization progress, including
%can confer significant benefits in terms of convergence rate 
a quick escape from plateaus.
%exploiting geometry-aware normalization), which escapes the plateaus quickly and  enjoys much faster convergence.

==> Non-uniform Smoothness/non_uniform_analysis.tex <==
% !TEX root = main_paper.tex

%\vspace{-2mm}
\section{Non-uniform Analysis}
\label{sec:non_uniform_analysis}

\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\linewidth]{figs/NS_Smoothness_diagram_table.pdf}
%\vskip -0.1in
\caption{Different function classes for $\beta(\theta^*) < \infty$. We use a label notation where, e.g., C denotes the set of all functions that satisfy property C, and $\text{ACE} \coloneqq \text{A} \cap \text{C} \cap \text{E}$. The two largest ellipsoids correspond to $\text{A} \cup \text{B}$ and C. We study the following four non-convex function classes in $( \text{A} \cup \text{B} ) \cap C$, i.e., $\gW \coloneqq \text{AC} \setminus ( \text{AD} \cup \text{ACE} )$, $\gX \coloneqq \text{AD} \setminus \text{ADE}$, $\gY \coloneqq \text{BC} \setminus ( \text{BD} \cup \text{BCE} )$, and $\gZ \coloneqq \text{BD} \setminus ( \text{BDE} \cup \text{BF} )$.
} 
\label{fig:non_uniform_function_classes_diagram_table}
%\vskip -0.2in
\end{figure*}

Our first main contribution is an analysis for GD and GNGD based in the presence of non-uniform properties. For minimization problems, we assume $\inf_{\theta}{ f(\theta) } > - \infty$ ($\sup_{\theta}{ f(\theta) } < \infty$ for maximization problems).
\begin{theorem}
\label{thm:general_optimization_main_result_1}
Suppose $f: \Theta \to \sR$ satisfies NS with $\beta(\theta)$ and 
the N\L{} inequality with $(C(\theta), \xi)$. 
Suppose $C \coloneqq \inf_{t \ge 1}{ C(\theta_t) } > 0$ for GD and GNGD. Let $\delta(\theta) \coloneqq f(\theta) - f(\theta^*)$ be the sub-optimality gap. The following hold:
%We have:
%Consider three cases:

\begin{description}[topsep=0pt,parsep=0pt]
%\item[(1)] The following hold:
%If $\beta(\theta) \to 0$ as $\theta, \theta^\prime \to \theta^*$ in \cref{def:non_uniform_smoothness}:

%Since $\delta(\theta)\!\to\!0$ and $\left\| \nabla f(\theta) \right\|_2\!\to\!0$ as $\theta\!\to\!\theta^*$, we have:
%\begin{description}[noitemsep, topsep=0pt,parsep=0pt]
\item[(1a)] if $\beta(\theta) \le c \cdot  \delta(\theta)^{1-2\xi}$ with $\xi \in (- \infty, 1/2)$, then the conclusions of (1b) hold;
\item[(1b)] if $\beta(\theta) \le c \cdot \left\| \nabla f(\theta) \right\|_2^{\frac{1 - 2 \xi}{1 - \xi}}$ with $\xi \in (- \infty, 1/2)$, then GD with $\eta \in O(1)$ achieves $\delta(\theta_t) \in  \Theta(1/t^{\frac{1}{1 - 2 \xi}})$,
and GNGD achieves $\delta(\theta_t) \in O(e^{- t})$.
%\end{description}
%
%\item[(2)] The following hold:
%If $\beta(\theta) \to \beta > 0$ as $\theta, \theta^\prime \to \theta^*$ in \cref{def:non_uniform_smoothness}:
%\begin{description}[noitemsep, topsep=0pt,parsep=0pt]
\item[(2a)] if $\beta(\theta) \le L_0 + L_1 \cdot \left\| \nabla f(\theta) \right\|_2$, then  the conclusions of (2b) hold;
\item[(2b)] if $\beta(\theta) \le L_0 \cdot \frac{\left\| \nabla f(\theta) \right\|^2}{ \delta(\theta)^{2 - 2 \xi} } + L_1 \cdot \left\| \nabla f(\theta) \right\|_2$, then GD and GNGD both achieve $\delta(\theta_t) \in O(1/t^{\frac{1}{1 - 2 \xi}})$ when $\xi \in (- \infty, 1/2)$, and $O(e^{-t})$ when $\xi = 1/2$. GNGD has strictly better constant than GD ($1 > C > C^2$).
%\end{description}
%
%\item[(3)]  The following hold:
%If $\beta(\theta) \to \infty$ as $\theta, \theta^\prime \to \theta^*$ in \cref{def:non_uniform_smoothness}:
%\begin{description}[noitemsep, topsep=0pt,parsep=0pt]
\item[(3a)] if $\beta(\theta)\!\le\!c\!\cdot\!\left\| \nabla f(\theta) \right\|_2^{\frac{1 - 2 \xi}{1 - \xi}}\!$ with $\xi \in (1/2, 1)$, then  the conclusions of (3b) hold;
\item[(3b)] if $\beta(\theta) \le c \cdot \delta(\theta)^{1 - 2 \xi}$ with $\xi \in (1/2, 1)$, then GD with $\eta \in \Theta(1)$ does not converge, while GNGD achieves $\delta(\theta_t) \in O(e^{-t})$.
%\end{description}
\end{description}
\end{theorem}

\begin{remark}
The cases (1)-(3) cover all three possibilities of $\beta(\theta^*)$. Since $\theta^*$ is the global minimum, $\nabla^2 f(\theta^*)$ is positive semi-definite (negative if $\theta^*$ is maximum) if it exists. 
\begin{itemize}[noitemsep, topsep=0pt,parsep=0pt]
	\item[(1)] If $\nabla^2 f(\theta^*) = \rvzero$, then $\beta(\theta) \to 0$ as $\theta, \theta^\prime \to \theta^*$, which means the landscape around $\theta^*$ is flat; 
	\item[(2)] If $\nabla^2 f(\theta^*)$ has at least one strictly positive (negative) eigenvalue, then $\beta(\theta) \to \beta > 0$ as $\theta, \theta^\prime \to \theta^*$. 
\end{itemize}
The cases (1)-(2) also cover the situations where the Hessian $\nabla^2 f(\theta^*)$ does not exist but one can find a finite $\beta(\theta^*) > 0$ to upper bound the l.h.s. of \cref{def:non_uniform_smoothness}. 
\begin{itemize}[noitemsep, topsep=0pt,parsep=0pt]
	\item[(3)] The case (3) is for blow-up type non-existence of $\nabla^2 f(\theta^*)$, where $\beta(\theta^*)$ is unbounded.
\end{itemize}
\end{remark}
\begin{remark}
In \cref{thm:general_optimization_main_result_1}, $C \coloneqq \inf_{t \ge 1}{ C(\theta_t) }$ is related to the early optimization and
plateau escaping behavior studied in \citet{mei2020escaping}. It remains open to study whether GNGD can be combined with different parameterizations in \citet{mei2020escaping} to further improve $C$.
\end{remark}

%\begin{remark}
Note that
(1b) recovers the strong smoothness of order $p$ with $p = 1 / \xi$ in \citet{wilson2019accelerating}, 
and (2a) recovers the $(L_0, L_1)$ smoothness of \citet{zhang2019gradient}. 
The results here consider more general N\L{} functions and establish faster rates of convergence. 
The other cases have not been studied in literature to our knowledge.
%\end{remark}
%
%\begin{remark}
In \cref{sec:policy_gradient,sec:generalized_linear_model} below we study practical machine learning examples that are covered by cases (1) and (2) in \cref{thm:general_optimization_main_result_1}. 
% There may other interesting applications for different cases of $\beta(\theta)$ and $\xi$ is left as future work, 
% We discuss related references about other special cases of $\beta(\theta)$ and $\xi$ in the appendix for completeness. 
Other cases of different $\beta(\theta)$ and $\xi$ are discussed in \cref{sec:proofs_non_uniform_analysis} for completeness.  
%\end{remark}

%\vspace*{-1mm}
\subsection{Function Classes and Existing Lower Bounds}
%\vspace*{-1mm}

Before applying these results to problems in machine learning, we first provide a refined characterization of function classes organized by their NS and N\L{} properties. 
This also clarifies the relation between the non-uniform properties and standard notions of convexity and smoothness; see \cref{fig:non_uniform_function_classes_diagram_table}. 
% and its correctness is given by the following propositions.

\begin{proposition}
\label{prop:function_class_relation}
The following %results 
hold for an objective $f$: 
\begin{itemize}[leftmargin=*,noitemsep, topsep=0pt,parsep=0pt]
\item[(1)] $\text{D} \subseteq \text{C}$. 
If %a function 
$f$ satisfies N\L{} with degree $\xi$, it satisfies N\L{} with degree $\xi^\prime < \xi$;
\item[(2)] $\text{F}\!\subseteq\!\text{D}$. 
A strongly convex %function 
$f$ satisfies N\L{} with $\xi\!=\!1/2$; 
\item[(3)] $\text{F} \cap \text{A} = \emptyset$. 
A strongly convex %function 
$f$ cannot satisfy NS with $\beta(\theta) \to 0$ as $\theta, \theta^\prime \to \theta^*$;
\item[(4)] $\text{E}\!\subseteq\!\text{C}$. 
A (not strongly) convex %function 
$f$ satisfies N\L{} with $\xi\!=\!0$.
\end{itemize}
\end{proposition}

The next proposition provides concrete examples for each convex function class in $(A \cup B) \cap C$ in \cref{fig:non_uniform_function_classes_diagram_table}.

\begin{proposition}
\label{prop:non_empty_convex_function_classes}
The following results hold: (1) $\text{ACE} \not= \emptyset$. (2) $\text{ADE} \not= \emptyset$. (3) $\text{BCE} \not= \emptyset$. (4) $\text{BDE} \not= \emptyset$. (5) $\text{BF} \not= \emptyset$.
\end{proposition}

A more interesting result considers examples in the classes of non-convex functions $(A \cup B) \cap C$ in \cref{fig:non_uniform_function_classes_diagram_table}. 
The non-uniform analysis above largely still applies to these %non-convex 
problems, even when standard convex analysis cannot apply.
\begin{proposition}
\label{prop:non_empty_non_convex_function_classes}
The following results hold: (1) $\gW \coloneqq \text{AC} \setminus ( \text{AD} \cup \text{ACE} ) \not= \emptyset$.  (2) $\gX \coloneqq \text{AD} \setminus \text{ADE} \not= \emptyset$. (3) $\gY \coloneqq \text{BC} \setminus ( \text{BD} \cup \text{BCE} ) \not= \emptyset$. (4) $\gZ \coloneqq \text{BD} \setminus ( \text{BDE} \cup \text{BF} ) \not= \emptyset$.
\end{proposition}
We next apply the techniques to a class of convex functions, 
achieving
%which provides 
results that cannot be explained by classical convex-smooth analysis.
\begin{proposition}
\label{prop:absulte_power_p}
    The convex function $f: x \mapsto |x|^p$ with $p > 1$ satisfies the N\L{} inequality with $\xi = 1/p$ and the NS property with $\beta(x) \le c_1 \cdot \delta(x)^{1 - 2 \xi}$.
\end{proposition}

Consider any $p > 2$, such as $p = 4$,
where it follows that $f$ satisfies N\L{} with degree $\xi = 1/4 < 1/2$. 
According to (1a) in \cref{thm:general_optimization_main_result_1}, GD will achieve $\delta(x_t) \in \Theta(1/t^2)$, while GNGD attains $\delta(x_t)\in O(e^{-c \cdot t})$ (where $c > 0$). 
Note that standard convex analysis can only give a $O(1/t)$ rate on (not strongly) convex smooth functions. 
The $\Theta(1/t^2)$ rate for GD here follows from using N\L{} degree $\xi = 1/4$, which improves on $\xi = 0$ from mere convexity 
((4) in \cref{prop:function_class_relation}). 
The $O(e^{-c \cdot t})$ rate has also been observed for this example by exploiting strong smoothness ((1b), as noted) \citep{wilson2019accelerating}.  \cref{fig:non_uniform_function_classes_diagram_table} provides a more general understanding of when this happens.

%\vspace{-3mm}
\paragraph{$\Omega(1/t^2)$ lower bound for convexity-smoothness.} 
Note that
GNGD satisfies $x_{t+1} = x_1 - \sum_{i=1}^{t}{ \frac{\eta}{\beta(x_i)} \cdot \nabla f(x_i) } \in \text{Span} \left\{x_1, \nabla f(x_1), \dots, \nabla f(x_t) \right\}$, which is a first-order oracle \citep{nesterov2003introductory}. 
%Therefore, 
Thus
there exists a worst-case objective in the convex-smooth class 
%for which %any first-order method cannot perform better than
that forces
$\delta(x_t)\in\Omega(1/t^2)$ for %sufficiently small 
$t \in O(n)$, where $n$ is the parameter dimension \citep{nemirovski1983problem,nesterov2003introductory,bubeck2014convex}. 
This is not a contradiction, since the
%There is no contradiction here. 
%The lower bound proof constructed 
%This classical 
lower bound is established by constructing
a convex smooth function with a \emph{constant} $\beta > 0$ \citep{bubeck2014convex}, and $\beta(x) \to \beta > 0$ as $x, x^\prime \to x^*$ in \cref{def:non_uniform_smoothness}. Hence, the $\Omega(1/t^2)$ result covers \textit{some} functions in BCE in \cref{fig:non_uniform_function_classes_diagram_table}. 
Meanwhile $f: x \mapsto |x|^p$ with $p > 2$ satisfies $\beta(x) \to 0$ as $x, x^\prime \to 0$ in \cref{def:non_uniform_smoothness} (ACE in \cref{fig:non_uniform_function_classes_diagram_table}),
which implies that the standard convex-smooth class consists of two subclasses. 
%Only one 
One
subclass (BCE) admits first-order sub-linear lower bounds, while the other %subclass 
(ACE) allows linear convergence using first-order methods. 
This illustrates the \emph{necessity} of non-uniformity in 
% This point of view is realizable after introducing the new NS property and 
subdividing the NS %function 
class as $\text{A} \cup \text{B}$ in \cref{fig:non_uniform_function_classes_diagram_table}.
This partition also inspires %the design of %the 
geometry-aware %first-order method 
GD.

% As shown in \cref{fig:non_uniform_function_classes_diagram_table}, subdividing the NS function classes goes beyond convexity-smoothness conditions, 
% Beyond the  convexity-smoothness conditions, there also exist lower bound results for $(L_0, L_1)$-smoothness.
%\vspace{-3mm}
\paragraph{$\Omega(1/\sqrt{t})$ lower bound for $(L_0, L_1)$-smoothness.} 
For $\beta(\theta) = L_0 + L_1 \cdot \| \nabla f(\theta) \|_2$ ((2a) in \cref{thm:general_optimization_main_result_1}) with $L_0, L_1 \ge 1$, standard normalized GD is subject to a $\Omega(1/\sqrt{t})$ lower bound \citep{zhang2019gradient}. However, in \cref{sec:policy_gradient}, we will show that normalized policy gradient (PG) method achieves a linear rate of $O(e^{- c \cdot t})$. 
%There is no contradiction, and the reason is similar. 
Again, this is not a contradiction for similar reasons.
With $L_0 \ge 1$, $\beta(\theta) \to L_0 > 0$ as $\theta, \theta^\prime \to \theta^*$,  
the $\Omega(1/\sqrt{t})$ lower bound will hold for \textit{some} functions in $\text{BCE} \cup \gY$ in \cref{fig:non_uniform_function_classes_diagram_table}.  While in \cref{sec:policy_gradient} the %policy value
objective satisfies $L_0 = 0$ and $L_1 > 0$, hence $\beta(\theta) \to 0$ as $\theta, \theta^\prime \to \theta^*$ ($\text{ACE} \cup \gW$ in \cref{fig:non_uniform_function_classes_diagram_table}). 
This shows a similar separation of rates for first-order methods will also occur based on NS conditions. 
Furthermore, in \cref{sec:generalized_linear_model}, we will show that both GD and GNGD achieve a $O(e^{- c \cdot t})$ rate for GLM,
but here the objective is in $\gZ$ in \cref{fig:non_uniform_function_classes_diagram_table} so the lower bounds do not apply.

%\vspace{-3mm}
\paragraph{Unbounded Hessian.} 
Consider any $p \in (1, 2)$, such as $p = 3/2$
where $f$ satisfies $\xi = 2 / 3$. 
According to \cref{thm:general_optimization_main_result_1}(3a), GD diverges since the Hessian is unbounded near $0$. 
This makes it \textit{necessary} to introduce geometry-aware normalization to ensure convergence, which is verified in \cref{sec:additional_simulations_experiments}.
%It has important practical implication 
This has practical implications for RL, 
for example ensuring exploration using state distribution entropy, which has unbounded Hessian near probability simplex boundary \citep{hazan2019provably} and alternative probability transforms \citep{mei2020escaping}.





==> Non-uniform Smoothness/non_uniform_properties.tex <==
% !TEX root = main_paper.tex

%\vspace{-2mm}
\section{Non-uniform Properties and Algorithms}
\label{sec:non_uniform_propterties}
%\vspace{-2mm}

The main results in this paper depend on
two core concepts, Non-uniform Smoothness (NS) and Non-uniform \L{}ojasiewicz (N\L{}) inequality.
The NS property is a new, intuitive generalization of smoothness. 
The N\L{} inequality is a recent proposal of \citet{mei2020global} and generalizes previous \L{}ojasiewicz inequalities.
% and recovers (strong) convexity as a special case. 
Our key contribution is to show that the \emph{combination} of these two non-uniform concepts is particularly powerful, applicable to important non-convex objectives in machine learning, and allows the development of improved algorithms and analysis. 

%\vspace{-2mm}
\subsection{Non-uniform Smoothness}

The first main concept we leverage is a generalized notion of smoothness that depends on the parameters non-uniformly.

%\vspace{-1mm}
\begin{definition}[Non-uniform Smoothness (NS)]
\label{def:non_uniform_smoothness}
The function $f: \Theta \to \sR$ satisfies $\beta(\theta)$ non-uniform smoothness if $f$ is differentiable and for all 
$\theta,\theta'\in\Theta$,
\begin{align*}
% \textstyle
    \left| f(\theta^\prime) - f(\theta) - \Big\langle \frac{d f(\theta)}{d \theta}, \theta^\prime - \theta \Big\rangle \right| \le \frac{{\color{red}\beta(\theta)}}{2} \cdot \| \theta^\prime - \theta \|_2^2,
\end{align*}
where $\beta$ is a positive valued function: $\beta: \Theta \to (0,\infty)$.
\end{definition}

We will refer to $\beta(\theta)$ in \cref{def:non_uniform_smoothness}  as the \textit{NS coefficient}. 
This alternative definition generalizes and unifies several smoothness concepts from the recent literature.
First, NS clearly reduces to \cref{eq:uniform smoothness} with $\beta(\theta) = \beta$. 
However, NS also generalizes the notion of $(L_0, L_1)$ smoothness from \citet{zhang2019gradient} by using $\beta(\theta) = L_0 + L_1 \cdot \left\| \nabla f(\theta) \right\|_2$. 
By using $\beta(\theta) = c \cdot \left\| \nabla f(\theta) \right\|_2^{\frac{p-2}{p-1}}$, NS also reduces to the notion of strong smoothness of order $p$ proposed in \citet{wilson2019accelerating}. 
Finally, with $\beta(\theta) = c / \left\| \theta \right\|_p^2$, NS reduces to a special form of non-uniform smoothness considered in \citet{mei2020escaping}. 
We will show later that NS also covers other previously unstudied smoothness variants. % that have not been previously studied.
%In \cref{sec:non_uniform_analysis,sec:policy_gradient,sec:generalized_linear_model} 
Below we will demonstrate the key benefits of \cref{def:non_uniform_smoothness} in terms of its \emph{generality}, \emph{better convergence results}, and \emph{practical implications}
in conjunction with the N\L{} inequality.

%\vspace{-2mm}
\subsection{Non-uniform \L{}ojasiewicz Inequality}

The second main concept we leverage is a generalized \L{}ojasiewicz inequality introduced by \citet{mei2020global}:

\begin{definition}[Non-uniform \L{}ojasiewicz (N\L{})]
\label{def:non_uniform_lojasiewicz}
The differentiable function $f : \Theta \to \sR$ satisfies the $(C(\theta), \xi)$ non-uniform \L{}ojasiewicz inequality if for all $\theta \in \Theta$,
\begin{align}
    \left\| \frac{ d f(\theta) }{d \theta} \right\|_2 \ge {\color{red}C(\theta)} \cdot \left| f(\theta) - f(\theta^*) \right|^{1-\xi},
\end{align}
where $\xi \in (-\infty, 1]$, and $C(\theta): \Theta \to \sR > 0$ holds for all $\theta \in \Theta$.
In this definition, either $\theta^*=\arg\min_{\theta\in\Theta}f(\theta)$,
or
$f(\theta^*)$ is replaced with $\inf_{\theta}{ f(\theta)}$ 
%or $\sup_{\theta}{ f(\theta)}$ 
if the global optimum is not achieved within the domain $\Theta$. 
\end{definition}
\cref{def:non_uniform_lojasiewicz} extends the classical ``uniform'' \L{}ojasiewicz inequalities in optimization literature, such as the Polyak-\L{}ojasiewicz (P\L{}) inequality with $C(\theta) = C > 0$ and $\xi = 1/2$ \citep{lojasiewicz1963propriete,polyak1963gradient}; and the Kurdyka-\L{}ojasiewicz (K\L{}) inequality\footnote{The K\L{} inequality is violated at bad local optima, since vanishing gradient norm cannot dominate non-zero sub-optimality gap. Therefore \cref{def:non_uniform_lojasiewicz} actually recovers global K\L{} inequality.} by setting $C(\theta) = C > 0$ \citep{kurdyka1998gradients}.
%
Following \citep{mei2020global,mei2020escaping}, we refer to $\xi$ as the \textit{N\L{} degree} and $C(\theta)$ as the \textit{N\L{} coefficient}.
Generally speaking, a larger N\L{} degree $\xi$ and N\L{} coefficient $C(\theta)$ indicate faster convergence for gradient based algorithms. 
\cref{sec:examples_non_convex_nl_inequality} provides an overview of remarkable non-convex functions that satisfy the N\L{} inequality for various $\xi$ and $C(\theta)$.
As stated, our main contribution in this paper is to show how,
when \emph{combined} with NS, N\L{} becomes a powerful tool for both algorithm design and analysis, which is a novel direction of investigation.


%This N\L{} inequality was first proposed in \citep{mei2020global} to analyze the convergence of policy gradient methods in reinforcement learning. 

% Generality is one advantage of using \cref{def:non_uniform_lojasiewicz}. 
%The major benefit of introducing non-uniformity is its generality. As mentioned before, for some non-convex optimization problems \citep{mei2020global}, it is not possible to find a uniform \L{}ojasiewicz inequality (where $C(\theta) = C > 0$), thus making it \textit{necessary} to use ``non-uniformity'' in  \cref{def:non_uniform_lojasiewicz}. 
%For references, we summarize existing non-convex functions that satisfy N\L{} inequalities to our knowledge in Appendix.


\subsection{Geometry-aware Gradient Descent}

A key benefit of the non-uniform definitions is that we can introduce stepsize 
rules that make gradient descent adapt to the local ``geometry'' of the optimization objective.
First consider the classical gradient decent update.

\begin{definition}[Gradient Descent (GD)]
\label{def:gd}
\begin{align}
\theta_{t+1} \gets \theta_t - \eta \cdot \nabla f(\theta_t).
\end{align}
\end{definition}

The key challenge with deploying GD is choosing the step size $\eta$;
if $\eta$ is too large, instability ensues,
if too small, progress becomes slow.
Recall from the introduction that $\eta=1/\beta$ is a canonical choice for assuring convergence in \emph{uniformly} $\beta$ smooth objectives.
This suggests that in the presence of \emph{non-uniform} smoothness $\beta(\theta)$ given in NS,
the stepsize should be adapted to $1/\beta(\theta)$. This leads to
 a new variant of normalized gradient descent.

\begin{definition}[Geometry-aware Normalized GD (GNGD)]
\label{def:gngd}
\begin{align}
\theta_{t+1} \gets \theta_t - \eta \cdot \frac{ \nabla f(\theta_t) }{ \color{red}{\beta(\theta_t)} }.
\end{align}
\end{definition}

Key to making this approach practical will be efficient ways to measure (or bound) $\beta(\theta)$.
Below we will show how in the context of NS and N\L{} properties, GNGD can be made both practical and extremely efficient at solving various 
global optimization problems in machine learning.
These results also broaden our fundamental knowledge of the set of objectives that admit efficient global optimization.

==> Non-uniform Smoothness/policy_gradient.tex <==
% !TEX root = main_paper.tex

\section{Policy Gradient}
\label{sec:policy_gradient}

Our second main contribution is to show that the expected return objective considered in direct policy optimization in RL %reinforcement learning (RL) 
falls under the %non-concave (due to maximization) 
function class $\gW$ in \cref{fig:non_uniform_function_classes_diagram_table}, in particular satisfying case (1) of   \cref{thm:general_optimization_main_result_1} with N\L{} degree $\xi = 0$. The key point is that value functions in Markov decision processes (MDPs) satisfy NS properties with coefficient being the PG norm (\cref{lem:non_uniform_smoothness_softmax_special,lem:non_uniform_smoothness_softmax_general}). This novel finding not only provides a much more precise characterization than existing standard smoothness results \citep{agarwal2020optimality,mei2020global}, but also enables PG with normalization to use the N\L{} inequalities (\cref{lem:non_uniform_lojasiewicz_softmax_special,lem:non_uniform_lojasiewicz_softmax_general}) differently than for standard PG ($\left\| \nabla f(\theta) \right\|_2$ vs. $\left\| \nabla f(\theta) \right\|_2^2$), which leads to faster convergence as well as plateau escaping.

\subsection{RL Settings and Notations}

For a finite set $\gN$, let $\Delta(\gN)$ denote the set of all probability distributions on $\gN$. A finite MDP $\gM \coloneqq (\gS, \gA, \gP, r, \gamma)$ is determined by a finite state space $\gS$, a finite action space $\gA$, a transition function $\gP: \gS \times \gA \to \Delta(\gS)$, a scalar reward function $r: \gS \times \gA \to \sR$, and a discount factor $\gamma \in [0 , 1)$. 

In policy-based RL, an agent interacts with the environment, i.e., the MDP $\gM$, using a policy $\pi: \gS \to \Delta(\gA)$. Given a state $s_t$, the agent takes an action $a_t \sim \pi(\cdot | s_t)$, receives a one-step scalar reward $r(s_t, a_t)$ and a next-state $s_{t+1} \sim \gP( \cdot | s_t, a_t)$. The long-term expected reward, also known as the value function of $\pi$ under $s$, is defined as
\begin{align}
\label{eq:state_value_function}
    V^\pi(s) \coloneqq \expectation_{\substack{s_0 = s, a_t \sim \pi(\cdot | s_t), \\ s_{t+1} \sim \gP( \cdot | s_t, a_t)}}{\left[ \sum_{t=0}^{\infty}{\gamma^t r(s_t, a_t)} \right]}.
\end{align}
The state-action value of $\pi$ at $(s,a) \in \gS \times \gA$ is defined as $Q^\pi(s, a) \coloneqq r(s, a) + \gamma \sum_{s^\prime}{ \gP( s^\prime | s, a) V^\pi(s^\prime) }$, and $A^\pi(s,a) \coloneqq Q^\pi(s, a) - V^\pi(s)$ is the advantage function of $\pi$.
The state distribution of $\pi$ is defined as,
\begin{align}
     d_{s_0}^{\pi}(s) \coloneqq (1 - \gamma) \sum_{t=0}^{\infty}{ \gamma^t \probability(s_t = s | s_0, \pi, \gP) }.
\end{align}
Given an initial state distribution $\rho \in \Delta(\gS)$, we denote $V^\pi(\rho) \coloneqq \expectation_{s \sim \rho}{ \left[ V^\pi(s) \right]}$ and $d_{\rho}^{\pi}(s) \coloneqq \expectation_{s_0 \sim \rho}{\left[ d_{s_0}^{\pi}(s) \right]}$. There exists an optimal policy $\pi^*$ such that $V^{\pi^*}(\rho) = \sup_{\pi : \gS \to \Delta(\gA) }{ V^{\pi}(\rho)}$. For convenience, we denote $V^* \coloneqq V^{\pi^*}$. 
Consider a tabular representation, i.e., $\theta(s,a) \in \sR$ for all $(s,a)$, so that the policy $\pi_\theta$ can be parameterized by $\theta$ as $\pi_\theta(\cdot | s) = \softmax(\theta(s, \cdot))$; 
that is, for all $(s,a)$,
\begin{align}
    \pi_\theta(a | s) = \frac{ \exp\{ \theta(s, a) \} }{ \sum_{a^\prime \in \gA}{ \exp\{ \theta(s, a^\prime) \} } }.
\end{align}
When there is only one state the policy $\pi_\theta = \softmax(\theta)$ is defined as $\pi_\theta(a) = \exp\{ \theta(a) \} / \sum_{a^\prime \in \gA}{ \exp\{ \theta(a^\prime) } $. The problem of policy-based RL is then to find a policy $\pi_\theta$ that maximizes the value function, i.e.,
\begin{align}
    \sup_{\theta : \gS \times \gA \to \sR}{ V^{\pi_\theta}(\rho) }. 
\end{align}
For convenience, and without loss of generality, we assume $r(s,a) \in [0, 1]$ for all $(s, a) \in \gS \times \gA$.

\subsection{One-state MDPs}

We first illustrate some key insights for  one-state MDPs with $K$ actions and $\gamma = 0$. The value function \cref{eq:state_value_function} reduces to expected reward $\pi_\theta^\top r$, where $r \in [0 ,1]^K$, $\theta \in \sR^K$, and $\pi_\theta = \softmax(\theta)$. 
\citet{mei2020global} have shown that even though $\max_{\theta}{ \pi_\theta^\top r}$ is a non-concave maximization, global convergence can be achieved with a $O(1/t)$ rate using uniform smoothness and the N\L{} inequality:

\begin{lemma}[N\L{}, \citet{mei2020global}, Lemma 3]
\label{lem:non_uniform_lojasiewicz_softmax_special}
Let $a^*$ be the optimal action.
Denote $\pi^* = \argmax_{\pi \in \Delta}{ \pi^\top r}$. Then, 
\begin{align}
    \left\| \frac{d \pi_\theta^\top r}{d \theta} \right\|_2 \ge \pi_\theta(a^*) \cdot ( \pi^* - \pi_\theta )^\top r.
\end{align}
\end{lemma}

Note that \cref{lem:non_uniform_lojasiewicz_softmax_special} is not improvable in terms of the coefficients $C(\theta) = \pi_\theta(a^*)$ and $\xi = 0$ \citep[Remark 1 and Lemma 17]{mei2020global}. 
However, this result is based on only using a \emph{uniform} smoothness coefficient $\beta = 5/2$ \citep[Lemma 2]{mei2020global}, which even empirical evidence suggests can be significantly refined.
To illustrate, we run standard policy gradient (PG) on a $3$-action one-state MDP. As shown in \cref{fig:expected_reward_non_uniform_smoothness}(a), PG first goes through a long suboptimal plateau, and then eventually escapes to approach $\pi^*$. \cref{fig:expected_reward_non_uniform_smoothness}(b) presents the spectral radius of the Hessian and the PG norm $3 \cdot \Big\| \frac{d \pi_{\theta_t}^\top r}{d \theta_t} \Big\|_2$ as functions of time $t$. 
It is evident that the smoothness behaves non-uniformly: it is close to zero at the suboptimal plateau and near $\pi^*$, highly aligned with the PG norm. 
Compared to any universal constant $\beta$, the PG  norm characterizes the non-uniform landscape information far more precisely. We formalize this observation by proving the following key result:
\begin{lemma}[NS]
\label{lem:non_uniform_smoothness_softmax_special}
Denote $\theta_\zeta\coloneqq \theta + \zeta \cdot (\theta^\prime - \theta)$ with some $\zeta\in [0,1]$. For any $r \in \left[ 0, 1\right]^K$, $\theta \mapsto \pi_\theta^\top r$ satisfies $\beta(\theta_\zeta)$ non-uniform smoothness with $\beta(\theta_\zeta) = 3 \cdot \Big\| \frac{d \pi_{\theta_\zeta}^\top r}{d {\theta_\zeta}} \Big\|_2 $.
\end{lemma}

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figs/expected_reward_non_uniform_smoothness.pdf}
%\vskip -0.1in
\caption{PG results on $r = (1.0, 0.8, 0.1)^\top$.} 
\label{fig:expected_reward_non_uniform_smoothness}
%\vskip -0.2in
\end{figure}

Comparing \cref{lem:non_uniform_smoothness_softmax_special} with (1b) in \cref{thm:general_optimization_main_result_1}, we have $\xi = 0$, and GNGD requires normalizing $\beta(\theta_\zeta)$, which is the PG norm of $\theta_\zeta$ rather than $\theta$. However, $\zeta$ is unknown. Fortunately, the next lemma shows that, if we still normalize the PG norm of $\theta$, the $\beta(\theta_\zeta)$ in \cref{lem:non_uniform_smoothness_softmax_special} can be upper bounded by $\Big\| \frac{d \pi_{\theta}^\top r}{d {\theta}} \Big\|_2$, given the learning rate is small enough:

\begin{lemma}
\label{lem:non_uniform_smoothness_intermediate_policy_gradient_norm_special}
Let $\theta^\prime = \theta + \eta \cdot \frac{d \pi_{\theta}^\top r}{d {\theta}} \Big/ \left\| \frac{d \pi_{\theta}^\top r}{d {\theta}} \right\|_2$. Denote $\theta_\zeta \coloneqq \theta + \zeta \cdot (\theta^\prime - \theta)$ with some $\zeta \in [0,1]$. We have, for all $\eta \in ( 0 , 1/3)$,
\begin{align}
    \bigg\| \frac{d \pi_{\theta_{\zeta}}^\top r}{d {\theta_{\zeta}}} \bigg\|_2 \le \frac{1}{1 - 3 \eta} \cdot \left\| \frac{d \pi_{\theta}^\top r}{d {\theta}} \right\|_2.
\end{align}
\end{lemma}

Next, the N\L{} coefficient $\pi_\theta(a^*)$ is bounded away from $0$, which provides constants in the convergence rate results.

\begin{lemma}[Non-vanishing N\L{} coefficient]
\label{lem:optimal_action_prob_positive}
\label{lem:lower_bound_cT_softmax_special}
Using normalized policy gradient method, we have $\inf_{t\ge 1} \pi_{\theta_t}(a^*) > 0$. 
\end{lemma}

To this point, we demonstrate that the non-concave function $\pi_\theta^\top r$ satisfies (1b) in \cref{thm:general_optimization_main_result_1} with $\xi = 0$ \textit{in each iteration of normalized PG}\footnote{This essentially means we prove that a uniform \L{}ojasiewicz inequality holds for the entire sequence $\left\{ \theta_t \right\}_{t\ge 1}$, but this does not
imply that the N\L{} condition is unnecessary. As shown in \citet[Remark 1]{mei2020global}, \L{}ojasiewicz-type inequalities with constant
$C > 0$ cannot hold. It can only become uniform after specifying an initialization $\theta_1$ and an algorithm (in this case, PG). Otherwise, uniform \L{}ojasiewicz cannot hold since initialization can make the N\L{}
coefficient $\pi_\theta(a^*)$ arbitrarily close to $0$.}: \cref{lem:non_uniform_smoothness_softmax_special,lem:non_uniform_smoothness_intermediate_policy_gradient_norm_special} show that the NS coefficient $\beta(\theta_{\zeta_t}) \le c_1 \cdot \Big\| \frac{d \pi_{\theta_t}^\top r}{d {\theta_t}} \Big\|_2$, while \cref{lem:non_uniform_lojasiewicz_softmax_special,lem:lower_bound_cT_softmax_special} guarantee $\Big\| \frac{d \pi_{\theta_t}^\top r}{d {\theta_t}} \Big\|_2 \ge c_2 \cdot ( \pi^* - \pi_{\theta_t} )^\top r$. Therefore, combining \cref{lem:non_uniform_smoothness_softmax_special,lem:non_uniform_lojasiewicz_softmax_special,lem:optimal_action_prob_positive,lem:non_uniform_smoothness_intermediate_policy_gradient_norm_special}, we prove the global linear convergence rate $O(e^{- c \cdot t})$ of normalized PG:

\begin{theorem}
\label{thm:final_rates_normalized_softmax_pg_special}
Using normalized PG $\theta_{t+1} = \theta_t + \eta \cdot \frac{d \pi_{\theta_t}^\top r}{d {\theta_t}} \Big/ \Big\| \frac{d \pi_{\theta_t}^\top r}{d {\theta_t}} \Big\|_2$, with $\eta = 1/6$, for all $t \ge 1$, we have, 
\begin{align}
    ( \pi^* - \pi_{\theta_t} )^\top r \le e^{ - \frac{  c \cdot (t-1) }{12} } \cdot \left( \pi^* - \pi_{\theta_{1}}\right)^\top r,
\end{align}
where $c = \inf_{t\ge 1} \pi_{\theta_t}(a^*) > 0$ is from \cref{lem:lower_bound_cT_softmax_special}, and $c$ is a constant that depends on $r$ and $\theta_1$, but not on the time $t$.
\end{theorem}

\begin{remark}
If $\pi_{\theta_1}$ is uniform, i.e., $\pi_{\theta_1}(a) = 1/K$, $\forall \ a \in [K]$, then we have $c \ge 1/K$ in \cref{thm:final_rates_normalized_softmax_pg_special}. This can be proved by showing that $\pi_{\theta_{t+1}}(a^*) \ge \pi_{\theta_{t}}(a^*)$, similar to \citet[Proposition 2]{mei2020global}.
\end{remark}


\subsection{Geometry-aware Normalized PG (GNPG)}

Next, we generalize from one-state to finite MDPs, using the GNPG\footnote{We use GNPG as the name of \cref{alg:normalized_policy_gradient_softmax}, since NPG is usually used to refer to the natural PG algorithm in RL literature.} on value function, as shown in \cref{alg:normalized_policy_gradient_softmax}.
\begin{algorithm}[ht]
   \caption{Geometry-aware Normalized Policy Gradient}
   \label{alg:normalized_policy_gradient_softmax}
\begin{algorithmic}
   \STATE {\bfseries Input:} Learning rate $\eta > 0$.
   \STATE Initialize parameter $\theta_1(s,a)$ for all $(s,a)$.
   \WHILE{$t \ge 1$}
   \STATE $\theta_{t+1} \gets \theta_{t} + \eta \cdot \frac{\partial V^{\pi_{\theta_t}}(\mu)}{\partial \theta_t} \Big/ \left\| \frac{\partial V^{\pi_{\theta_t}}(\mu)}{\partial \theta_t} \right\|_2 $.
%   \STATE Perform policy evaluation to obtain $V^{\pi_{\theta_{t+1}}}(\mu)$
   \ENDWHILE
\end{algorithmic}
\end{algorithm}

\subsection{General MDPs}

For general finite MDPs, we assume ``sufficient exploration'' for the initial state distribution $\mu$, which is also adapted in literature \citep{agarwal2020optimality,mei2020global}.

\begin{assumption}[Sufficient exploration]\label{ass:posinit}
The initial state distribution satisfies $\min_s \mu(s)>0$.
\end{assumption}

Given \cref{ass:posinit}, \citet{agarwal2020optimality} prove asymptotic global convergence for PG on the non-concave $\max_{\theta}{ V^{\pi_\theta}(\rho)}$ problem,
while \citet{mei2020global} strengthens this to a $O(1/t)$ rate using uniform smoothness and the following N\L{} inequality that generalizes \cref{lem:non_uniform_lojasiewicz_softmax_special}.

\begin{lemma}[N\L{}, \citet{mei2020global}, Lemma 8] Denote $S \coloneqq | \gS| $ as the total number of states. We have, $\forall \ \theta \in \sR^{\gS \times \gA}$,
\label{lem:non_uniform_lojasiewicz_softmax_general}
\begin{align*}
    \left\| \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta }\right\|_2 \ge \frac{ \min_s{ \pi_\theta(a^*(s)|s) } }{ \sqrt{S} \cdot  \left\| d_{\rho}^{\pi^*} / d_{\mu}^{\pi_\theta} \right\|_\infty } \cdot \left( V^*(\rho) - V^{\pi_\theta}(\rho) \right),
\end{align*}
where $a^*(s)$ is the action that $\pi^*$ selects in state $s$.
\end{lemma}

Here, the N\L{} degree $\xi = 0$ is not improvable \citet[Lemma 28]{mei2020global}. In one-state MDPs with $S = 1$, \cref{lem:non_uniform_lojasiewicz_softmax_general} recovers \cref{lem:non_uniform_lojasiewicz_softmax_special} with the same N\L{} coefficient $C(\theta) = \pi_\theta(a^*)$, indicating that $C(\theta)$ in \cref{lem:non_uniform_lojasiewicz_softmax_general} might also be unimprovable. On the other hand, the uniform smoothness considered in \citep{agarwal2020optimality,mei2020global} $\beta = 8 / (1 - \gamma)^3$ is too conservative, particularly when $\gamma$ is close to $1$. Our next key result shows that the policy value also satisfies a stronger NS property, with the NS coefficient being the PG norm, generalizing \cref{lem:non_uniform_smoothness_softmax_special}:
\begin{lemma}[NS]
\label{lem:non_uniform_smoothness_softmax_general}
Let \cref{ass:posinit} hold and denote $\theta_\zeta \coloneqq \theta + \zeta \cdot (\theta^\prime - \theta)$ with some $\zeta \in [0,1]$. $\theta \mapsto V^{\pi_\theta}(\mu)$ satisfies $\beta(\theta_\zeta)$ non-uniform smoothness with
\begin{align*}
    \beta(\theta_\zeta) = \left[ 3 + \frac{ 4 \cdot \left( C_\infty - (1 - \gamma) \right) }{ 1 - \gamma } \right] \cdot \sqrt{S} \cdot \left\| \frac{\partial V^{\pi_{\theta_\zeta}}(\mu)}{\partial {\theta_\zeta} }\right\|_2,
\end{align*}
where $C_\infty \coloneqq \max_{\pi}{ \left\| \frac{d_{\mu}^{\pi}}{ \mu} \right\|_\infty} \le \frac{1}{ \min_s \mu(s) } < \infty$.
\end{lemma}
In one-state MDPs with $\gamma = 0$ and $S = 1$, we have $C_\infty = 1 - \gamma$. Thus \cref{lem:non_uniform_smoothness_softmax_general} reduces to \cref{lem:non_uniform_smoothness_softmax_special} with the same NS coefficient $\beta(\theta_\zeta) = 3 \cdot \Big\| \frac{d \pi_{\theta_\zeta}^\top r}{d {\theta_\zeta}} \Big\|_2$. Similar to \cref{lem:non_uniform_smoothness_intermediate_policy_gradient_norm_special}, if we use \cref{alg:normalized_policy_gradient_softmax} with small enough learning rate, then $\beta(\theta_\zeta)$ in \cref{lem:non_uniform_smoothness_softmax_general} is upper bounded by the PG norm of $\theta$:
\begin{lemma}
\label{lem:non_uniform_smoothness_intermediate_policy_gradient_norm_general}
Let $\eta = \frac{1 - \gamma }{ 6 \cdot ( 1 - \gamma)  + 8 \cdot \left( C_\infty - (1 - \gamma) \right) } \cdot \frac{ 1}{ \sqrt{S} }$ and $\theta^\prime = \theta + \eta \cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta} \Big/ \left\| \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta} \right\|_2$. Denote $\theta_\zeta \coloneqq \theta + \zeta \cdot (\theta^\prime - \theta)$ with some $\zeta \in [0,1]$. We have,
\begin{align}
%\textstyle
    \left\| \frac{\partial V^{\pi_{\theta_\zeta}}(\mu)}{\partial \theta_\zeta} \right\|_2 \le 2 \cdot \left\| \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta} \right\|_2.
\end{align}
\end{lemma}
Next, the N\L{} coefficient $\min_s{ \pi_\theta(a^*(s)|s) }$ in \cref{lem:non_uniform_lojasiewicz_softmax_general} is lower bounded away from $0$:
\begin{lemma}[Non-vanishing N\L{} coefficient]
\label{lem:lower_bound_cT_softmax_general}
Let \cref{ass:posinit} hold. We have,
$c:=\inf_{s\in \cS,t\ge 1} \pi_{\theta_t}(a^*(s)|s) > 0$, where $\left\{ \theta_t \right\}_{t\ge 1}$ is generated by \cref{alg:normalized_policy_gradient_softmax}.
\end{lemma}
Now we have the non-concave function $V^{\pi_\theta}(\rho)$ satisfies (1b) in \cref{thm:general_optimization_main_result_1} with $\xi = 0$ \textit{in each iteration of \cref{alg:normalized_policy_gradient_softmax}}. Therefore, combining \cref{lem:non_uniform_smoothness_softmax_general,lem:non_uniform_lojasiewicz_softmax_general,lem:lower_bound_cT_softmax_general,lem:non_uniform_smoothness_intermediate_policy_gradient_norm_general}, we prove the global linear convergence rate $O(e^{-c \cdot t})$ of \cref{alg:normalized_policy_gradient_softmax}:
\begin{theorem}
\label{thm:final_rates_normalized_softmax_pg_general}
Let \cref{ass:posinit} hold and
let $\left\{ \theta_t \right\}_{t\ge 1}$ be generated using  \cref{alg:normalized_policy_gradient_softmax} with $\eta = \frac{ 1 - \gamma }{ 6 \cdot ( 1 - \gamma)  + 8 \cdot \left( C_\infty - (1 - \gamma) \right) } \cdot \frac{ 1}{ \sqrt{S} }$, where $C_\infty \coloneqq \max_{\pi}{ \left\| \frac{d_{\mu}^{\pi}}{ \mu} \right\|_\infty}$. Denote $C_\infty^\prime \coloneqq \max_{\pi}{ \left\| \frac{d_{\rho}^{\pi}}{ \mu} \right\|_\infty}$. Let $c$ be the positive constant from \cref{lem:lower_bound_cT_softmax_general}.
We have, for all $t\ge 1$,
\begin{align*}
    V^*(\rho) - V^{\pi_{\theta_t}}(\rho) \le \frac{ \left( V^*(\mu) - V^{\pi_{\theta_1}}(\mu) \right) \cdot C_\infty^\prime }{ 1 - \gamma} \cdot e^{ - C \cdot (t-1)},
\end{align*}
where $C = \frac{ ( 1 - \gamma)^2 \cdot c }{ 12 \cdot ( 1 - \gamma)  + 16 \cdot \left( C_\infty - (1 - \gamma) \right) } \cdot \frac{ 1}{ S } \cdot \Big\| \frac{d_{\mu}^{\pi^*}}{\mu} \Big\|_\infty^{-1} $.
\end{theorem}
Not only the $O(e^{-c \cdot t})$ rate in \cref{thm:final_rates_normalized_softmax_pg_general} is faster than $O(1/t)$ for standard PG without normalization, but also the constant is better than \citet[Theorem 4]{mei2020global}. The strictly better dependence $c$ ($\gg c^2$ in PG) is related to faster escaping plateaus as shown later \citep{mei2020escaping}. 
\begin{remark}
The conclusion of GNPG has better constants than PG ($c \gg c^2$) arises from upper bounds (\cref{thm:final_rates_normalized_softmax_pg_general} and \citet[Theorem 4]{mei2020global}), which is also supported by empirical evidence. In fact, there exists a lower bound that shows $c$ cannot be removed for PG \citep[Theorem 1]{mei2020escaping} under one-state MDP settings. For finite MDPs, very recently, \citet{li2021softmax} show that for softmax PG (without normalization), $c$ can be very small in terms of the number of states. It remains open to consider whether $c$ is reasonably large for GNPG.
\end{remark}
\begin{remark}
To our knowledge, existing PG variants can achieve linear convergence $O(e^{-c \cdot t})$ only if using at least one of the following techniques: (a) \textbf{regularization}; \citet{mei2020global} prove that entropy regularized PG enjoys $O(e^{-c \cdot t})$ convergence toward the regularized optimal policy. (b) \textbf{natural gradient}; \citet{cen2020fast} prove that entropy regularized natural PG achieves linear convergence. (c) \textbf{exact line-search}; \citet{bhandari2020note} prove that without parameterization, PG variants with exact line-search achieve linear rates by approximating policy iteration.



\if0
On the other hand, without using any above technique, the best known convergence rate of policy gradient methods was $O(1/t)$ \citep{agarwal2020optimality,mei2020global}.
\fi

Among the above techniques, regularization changes the problem to regularized MDPs, while natural PG and line-search require solving expensive optimization problems to do updates, since each update is an $\argmax$.
\end{remark}
On the contrary, \cref{alg:normalized_policy_gradient_softmax} enjoys global $O(e^{-c \cdot t})$ rate \textit{(i)} without using regularization, since \cref{alg:normalized_policy_gradient_softmax} directly works on the original MDPs; \textit{(ii)} without solving optimization problems in each iteration, and the normalized PG update is cheap. The strong results rely on the NS and N\L{} properties, and also the geometry-aware normalization that takes advantage of the non-uniform properties.
\begin{remark}
Standard softmax PG with bounded learning rate follows $\Omega(1/t)$ lower bound \citep{mei2020global}, which is consistent with the case (1) in \cref{thm:general_optimization_main_result_1}. \cref{alg:normalized_policy_gradient_softmax} achieves faster  linear convergence rates, indicating that the adaptive update stepsize $\eta / \left\| \nabla V^{\pi_{\theta_t}}(\rho) \right\|_2$ is asymptotically unbounded, since $\left\| \nabla V^{\pi_{\theta_t}}(\rho) \right\|_2 \to 0$ as $t \to \infty$.
\end{remark}
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figs/pg_npg_expected_reward_sub_optimality.pdf}
%\vskip -0.1in
\caption{PG and GNPG on $r = (1.0, 0.8, 0.1)^\top$.} 
\label{fig:pg_npg_expected_reward_sub_optimality}
%\vskip -0.2in
\end{figure}
We compare PG and GNPG on the one-state MDP problem as shown in \cref{fig:pg_npg_expected_reward_sub_optimality}. \cref{fig:pg_npg_expected_reward_sub_optimality}(a) shows that GNPG escapes from the sub-optimal plateau significantly faster than PG, while \cref{fig:pg_npg_expected_reward_sub_optimality}(b) shows that GNPG follows linear convergence $O(e^{-c \cdot t})$ of sub-optmality, verifying the theoretical results. Similar experimental results on synthetic tree MDPs with multiple states are presented in \cref{sec:additional_simulations_experiments}.

